Searches for rare and non-Standard Model decays of the Higgs boson

Discovered in 2012, the Higgs boson has opened a new window on nature. The latest searches for its rare and non-Standard Model decays with the ATLAS detector at the LHC are presented. They represent a promising probe of the 1st and 2nd generation Yukawa couplings, and of new physics. Searches for rare exclusive decays of the Higgs boson to a meson and a photon are presented. Also presented are four searches for decays of the Higgs boson to pairs of beyond the Standard Model resonances, in various final states.

==> Makefile <==
filename=RareOrBSMHiggsDecays_CIPANP2018_ElliotReynolds_Proceedings

default:
	pdflatex ${filename}.tex
	pdflatex ${filename}.tex

clean:
	rm -f ${filename}.{ps,pdf,log,aux,out,dvi,bbl,blg,toc,nav,snm}
	find figures -name "*-eps-converted-to.pdf" -exec rm -f {} \;

